Beer Mats make bad Frisbees

In this article we show why flying and rotating beer mats, CDs, or other flat disks will eventually flip in the air and end up flying with backspin, thus, making them unusable as frisbees. The crucial effect responsible for the flipping is found to be the lift attacking not in the center of mass but slightly offset to the forward edge. This induces a torque leading to a precession towards backspin orientation. An effective theory is developed providing an approximate solution for the disk's trajectory with a minimal set of parameters. Our theoretical results are confronted with experimental results obtained using a beer mat shooting apparatus and a high speed camera. Very good agreement is found.

==> figures/y_t_10000_zu_0_hinten.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  % Encoding inside the plot.  In the header of your document, this encoding
  % should to defined, e.g., by using
  % \usepackage[latin1,<other encodings>]{inputenc}
  \inputencoding{latin1}%
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3772.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}$-0.6$}}%
      \csname LTb\endcsname%%
      \put(946,1111){\makebox(0,0)[r]{\strut{}$-0.5$}}%
      \csname LTb\endcsname%%
      \put(946,1517){\makebox(0,0)[r]{\strut{}$-0.4$}}%
      \csname LTb\endcsname%%
      \put(946,1924){\makebox(0,0)[r]{\strut{}$-0.3$}}%
      \csname LTb\endcsname%%
      \put(946,2331){\makebox(0,0)[r]{\strut{}$-0.2$}}%
      \csname LTb\endcsname%%
      \put(946,2738){\makebox(0,0)[r]{\strut{}$-0.1$}}%
      \csname LTb\endcsname%%
      \put(946,3144){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(946,3551){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \csname LTb\endcsname%%
      \put(1078,484){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(1474,484){\makebox(0,0){\strut{}$0.1$}}%
      \csname LTb\endcsname%%
      \put(1870,484){\makebox(0,0){\strut{}$0.2$}}%
      \csname LTb\endcsname%%
      \put(2266,484){\makebox(0,0){\strut{}$0.3$}}%
      \csname LTb\endcsname%%
      \put(2662,484){\makebox(0,0){\strut{}$0.4$}}%
      \csname LTb\endcsname%%
      \put(3059,484){\makebox(0,0){\strut{}$0.5$}}%
      \csname LTb\endcsname%%
      \put(3455,484){\makebox(0,0){\strut{}$0.6$}}%
      \csname LTb\endcsname%%
      \put(3851,484){\makebox(0,0){\strut{}$0.7$}}%
      \csname LTb\endcsname%%
      \put(4247,484){\makebox(0,0){\strut{}$0.8$}}%
      \csname LTb\endcsname%%
      \put(4643,484){\makebox(0,0){\strut{}$0.9$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2127){\rotatebox{-270}{\makebox(0,0){\strut{}$y/m$}}}%
      \put(2860,154){\makebox(0,0){\strut{}$t/s$}}%
      \csname LTb\endcsname%%
      \put(1738,1097){\makebox(0,0)[r]{\strut{}data}}%
      \csname LTb\endcsname%%
      \put(1738,877){\makebox(0,0)[r]{\strut{}fit}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{y_t_10000_zu_0_hinten-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> sections/theory.tex <==
\section{Forces and Equations of Motions}

The movement of a freely moving rigid body can be described using six coordinates: the position $\vec x = (x,y,z)$, the polar angle $\theta$, the azimuth $\phi$ and the proper rotation $\psi$, see also Figure~\ref{fig_disk_sketch}. Newton's second law yields
\begin{equation}
	\vec F = m \ddot{\vec x} - m \vec g,
\end{equation}
a differential equations governing the movement of the center of mass, where $m$ is the mass of the disk, $\vec g$ is the gravitational acceleration and and $\vec F$ are the aerodynamic forces acting on the center of mass. Using Euler's equations or Lagrange's mechanics one can derive the equations
\begin{align}
 M_\theta ={}& I (\ddot\theta + \dot\phi^2 \cos\theta \sin\theta + 2\dot\phi\dot\psi\sin\theta) \\
 \begin{split} M_\phi ={}& I (\ddot\phi (1+\cos^2\theta) - 2\dot\theta\dot\phi\cos\theta\sin\theta \\&+ 2\ddot\psi\cos\theta - 2\dot\theta\dot\psi\sin\theta) \end{split}\\
 M_\psi ={}& I (\ddot\psi + 2\ddot\phi\cos\theta - \dot\theta\dot\phi\sin\theta)
\end{align}
%\begin{equation}
%	\vec M = \begin{pmatrix} M_\theta \\ M_\phi \\ M_\psi \end{pmatrix} \\= I \begin{pmatrix} \ddot\theta + \dot\phi^2 \cos\theta \sin\theta + 2\dot\phi\dot\psi\sin\theta \\ \ddot\phi (1+\cos^2\theta) - 2\dot\theta\dot\phi\cos\theta\sin\theta + 2\ddot\psi\cos\theta - 2\dot\theta\dot\psi\sin\theta \\ \ddot\psi + 2\ddot\phi\cos\theta - \dot\theta\dot\phi\sin\theta \end{pmatrix},
%\end{equation}
to describe the behaviour of $\theta$, $\phi$ and $\psi$. $\vec M = (M_\theta, M_\phi, M_\psi)$ denotes the torques acting on the disk and the moment of inertia tensor of the disk along its principal axes is $\operatorname{diag}(I,I,2I)$ with $I=\frac14 mr^2$.

Setting $\vec F=0$ and $\vec M=0$ would describe the disk's motion in vacuo, but since we are interested in the behaviour in air, the left hand sides of these six equations of motions need to be elaborated.


\subsection{Turbulent drag}

Generally turbulent drag acts proportionally to the fluid density $\rho$, the area $A$ of the object and its squared velocity. It is always working in the direction opposite to the velocity. We write
\begin{align}
	\vec F_\mathrm{drag} &= -\frac12 \rho c_\mathrm{drag}(\alpha) A |\vec v| \vec v,\\
	c_\mathrm{drag}(\alpha) &= c_0 + c_\mathrm{\alpha} \sin^2 \alpha \quad\text{and}\\
	\alpha &= \frac\pi2 - \arccos \frac{\vec v \cdot \vec d}{|\vec v|}.
\end{align}
Here $\alpha$ is the angle of attack, i.e. the angle between the leading edge of the disk and it's direction of movement. blabla the c's.

\subsection{Lifting force}

Schlichting/Truckenbrodt: Aerodynamik des Flugzeuges (Teil I), 1967, (2.203)

\begin{align}
	\vec F_\mathrm{lift} &= \frac12 \rho c_\mathrm{lift}(\alpha) A |\vec v|^2 \vec e_\mathrm{\perp \vec v},\\
	c_\mathrm{lift} &= 2\pi\sin\alpha \quad\text{for}\quad \alpha > 6^\circ.
\end{align}

\subsection{Lift induced torque}

(2.210)

\begin{align}
	M &= \frac12 \rho c_\mathrm{torque}(\alpha) A |\vec v|^2 \ell,\\
	c_\mathrm{torque} &= -\frac\pi4 \sin 2\alpha.
\end{align}

\subsection{}
\subsection{}

